Importance Weighting Approach in Kernel Bayes' Rule

We study a nonparametric approach to Bayesian computation via feature means, where the expectation of prior features is updated to yield expected kernel posterior features, based on regression from learned neural net or kernel features of the observations. All quantities involved in the Bayesian update are learned from observed data, making the method entirely model-free. The resulting algorithm is a novel instance of a kernel Bayes' rule (KBR), based on importance weighting. This results in superior numerical stability to the original approach to KBR, which requires operator inversion. We show the convergence of the estimator using a novel consistency analysis on the importance weighting estimator in the infinity norm. We evaluate KBR on challenging synthetic benchmarks, including a filtering problem with a state-space model involving high dimensional image observations. Importance weighted KBR yields uniformly better empirical performance than the original KBR, and competitive performance with other competing methods.

==> dataset_desc.tex <==
In this appendix, we briefly describe the image dataset we used in the experiments.

In the first experiment, we used DeepMind Lab dataset \citep{DeepMindLab}, which is originally designed for evaluating reinforcement learning agents. This platform provides a first-person viewpoint through the eyes of the agent, which can move freely in the maze. Based on this platform, we generate samples of rotating views of the agent who standing at the specific point in in the maze. The example of the image is shown in \cref{fig:dSprite-sample}
\begin{figure}
\begin{minipage}{0.4\columnwidth}
   \centering
   \includegraphics[width=\linewidth]{img/maze_example.png}
    \caption{DeepMind Lab} \label{fig:maze-sample}
  \end{minipage}
\hfill
\begin{minipage}{0.4\columnwidth}
   \centering
    \includegraphics[width=\linewidth]{img/dsprite_example.png}
    \caption{dSprite} \label{fig:dSprite-sample}
  \end{minipage}
\end{figure}


For another experiment,  we used dSprite \citep{dsprites}, which is a dataset of 2D shape images as shown in \cref{fig:dSprite-sample}. This is an image dataset described by five latent parameters ({\tt shape,  scale, rotation, posX} and {\tt posY}). The images are $64 \times 64 = 4096$-dimensional. 
